Search-Based Motion Planning for Performance Autonomous Driving

Driving on the limits of vehicle dynamics requires predictive planning of future vehicle states. In this work, a search-based motion planning is used to generate suitable reference trajectories of dynamic vehicle states with the goal to achieve the minimum lap time on slippery roads. The search-based approach enables to explicitly consider a nonlinear vehicle dynamics model as well as constraints on states and inputs so that even challenging scenarios can be achieved in a safe and optimal way. The algorithm performance is evaluated in simulated driving on a track with segments of different curvatures.

==> macros/packages.tex <==
%============================================================================
% The following packages can be found on http:\\www.ctan.org
% BIBTEX
\usepackage{cite}
% BIBLATEX: \usepackage[style=IEEEtran,backend=bibtex]{biblatex}

\usepackage{graphicx}  % for pdf, bitmapped graphics files
\usepackage{array}
%\usepackage{epsfig}   % for postscript graphics files
%\usepackage{mathptmx} % assumes new font selection scheme installed
\usepackage{times}     % assumes new font selection scheme installed
\usepackage[fleqn]{amsmath}   % assumes amsmath package installed
\usepackage{amssymb}   % assumes amsmath package installed
%\usepackage{mathabx}   % for \widebar % Böse (font 3)
\usepackage{dsfont}
\usepackage{float}     % for placing with (H) at a specific position 
\usepackage{textgreek}
\usepackage[table]{xcolor}  % Färbige Tabellen
\usepackage{booktabs}       % Schöne Tabellen (dicke und dünne Linien)
\usepackage{filemod}        % für autoupdate bei geänderten tikz-grafiken
\usepackage{xifthen}
\usepackage[linesnumbered,ruled,vlined]{algorithm2e}
\usepackage{epstopdf}
\usepackage{subcaption}
\usepackage{paralist}
\usepackage{footnote}
%==============================================================================
% macro for executing a shell command immidiatly 
%\newcommand{\runmycommand}[1]{\immediate\write18{#1}}
% AUTOMATIC BIBTEX
\IfFileExists{\jobname.aux}% needs --enable-write18
             {\typeout{bibtex \jobname.aux}
              \immediate\write18{bibtex \jobname.aux}
              \typeout{*** AUTO RUNNING BIBTEX ***}}
             {\typeout{*********** Rerun for bibliography *************}}
%FOR BIBLATEX %\addbibresource{./IEEEabrv,./library}
             
% Pakete für Blockdiagramme und Diagramme
\usepackage{tikz}               % Achtung die Reihenfolge der Tikz Pakete ist
\usepackage{pgfplots}           % entscheidend!
\usepackage{pgfplotstable} 
\usepgfplotslibrary{groupplots}
\usepgfplotslibrary{units}
%\usetikzlibrary{spy}
\usetikzlibrary{shadows,positioning,arrows}
%\usetikzlibrary{shapes,shapes.multipart}
\usetikzlibrary{calc}
\usetikzlibrary{trees,fit,backgrounds}
%\usetikzlibrary{patterns,decorations.pathreplacing,decorations.pathmorphing}
%\usetikzlibrary{decorations.markings}
\usetikzlibrary{matrix}
\usetikzlibrary{shadows.blur,shapes.symbols}

%=================================================================================
\usepgfplotslibrary{external} % PDFs machen
\tikzexternalize[prefix=tikz_temp/]     % Unterordner für PDFs
\newcommand\autoupdateexternfigure[2]{  % MAKRO UM AUTOUPDATE ZU ERMÖGLICHEN
  \tikzsetnextfilename{#2}              % pdf-filename
  \filemodCmp{#1}{tikz_temp/#2.log}%    % prüft file datum 
  {\tikzset{external/force remake=true}}% erzwingt remake wenn log alt
  {}
}
%\tikzset{external/force remake} % immer alle Bilder neu machen
% Achtung für später: EPS-Grafiken können mit Tikz auch automatisch erstellt werden (siehe Internet)
% Tipps zu eps: auf http://tex.stackexchange.com/questions/8641/export-eps-figures-from-tikz
%=================================================================================

% Spezial Worttrennungen
\hyphenation{Last-rampen Betriebs-punkt}

%============================================================================
% PDF-Einstellungen
%\usepackage[ pdfauthor={Zlatan Ajanovic, Michael Stolz, Martin Horn}
%             ,pdftitle={A Novel Observer Concept for Embedded Drivetrain Applications}
%             ,pdfpagelayout=TwoPageLeft
%             ,pdfstartview  = {FitV}
%             %,pdfpagemode  = UseAttachments %OPEN ATTACHMENTS-VIEW IN PD
%             ,pdfpagelabels = true
%             ,linkcolor     = {black}
%             ,colorlinks    = {true} 
%             ,citecolor     = {black}
%             ,urlcolor      = {black}
%             ,bookmarks, bookmarksnumbered
%             %,bookmarksopen={true}, 
%             %,pagebackref  = true, backref = page     %% turn on backreferencing
%             ,plainpages    = false
%             ,hypertexnames = true
%             ]{hyperref}
%============================================================================
% Matrizen ------------------------------------------------------------------  
%\usepackage{arydshln}         % have dotted lines to separate matrix elements 
%\newcommand{\myhdots}{\hdashline[.4pt/1.5pt]}          % macro für punktierte

==> macros/tikzStyles.tex <==
\tikzstyle{s} = [font = \footnotesize]

\tikzstyle{doppelpfeil} = [-latex,postaction={draw,shorten >=6pt,-latex}]
\tikzstyle{sarrowtip} = [>=latex]  
\tikzstyle{myarrowtip} = [>=implies] 

\tikzset{curveinscope/.style={every path/.style={draw=white, double distance=1pt, line width=2pt, double=black, text=black}}}

\DeclareRobustCommand{\myLine}[1]{
(\tikzset{external/export next=false}\begin{tikzpicture}%
\useasboundingbox (-0.2ex,0) rectangle (4.65ex,1ex);%
\draw[line width=0.3ex,#1](0,0.65ex)--(4.5ex,0.65ex);%
\end{tikzpicture})}



